QSO MUSEUM I: A sample of 61 extended Ly$\alpha$-emission nebulae surrounding $z\sim3$ quasars

Motivated by the recent discovery of rare Enormous Lyman-Alpha Nebulae (ELAN) around z~2 quasars, we have initiated a long-term observational campaign with the MUSE instrument to directly uncover the astrophysics of the gas around quasars. We present here the first 61 targets of our effort under the acronym QSO MUSEUM (Quasar Snapshot Observations with MUse: Search for Extended Ultraviolet eMission). These quasars have a median redshfit of z=3.17, absolute $i$ magnitude in the range $-29.67\leq M_i(z=2)\leq-27.03$, and different levels of radio-loudness. This sample unveils diverse specimens of Ly$\alpha$ nebulosities extending for tens of kiloparsecs around these quasars (on average out to a maximum projected distance of 80 kpc) above a surface brightness SB$>8.8\times10^{-19}$ erg s$^{-1}$ cm$^{-2}$ arcsec$^{-2}$ ($2\sigma$). The bulk of the extended Ly$\alpha$ emission is within R<50 kpc, and is characterized by relatively quiescent kinematics, with average velocity dispersions of $\langle \sigma_{\rm Ly\alpha}\rangle < 400$~km~s$^{-1}$. Therefore, the motions within all these Ly$\alpha$ nebulosities have amplitudes consistent with gravitational motions expected in dark matter halos hosting quasars at these redshifts, possibly reflecting the complexity in propagating a fast wind on large scales. Our current data suggest a combination of photoionization and resonant scattering as powering mechanisms of the Ly$\alpha$ emission. We discover the first $z\sim3$ ELAN, which confirms a very low probability ($\sim1\%$) of occurrence of such extreme systems at these cosmic epochs. Finally, we discuss the redshift evolution currently seen in extended Ly$\alpha$ emission around radio-quiet quasars from $z\sim3$ to $z\sim2$, concluding that it is possibly linked to a decrease of cool gas mass within the quasars' CGM from $z\sim3$ to $z\sim2$, and thus to the balance of cool vs hot media.

==> Tab_LAEs_6dFJ0032-0414.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around 6dFJ0032-0414 (or ID=48).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  00:32:05.856    &  -04:14:15.02    & 8.5	      & 5048.68$\pm$0.03 & 3.153$\pm$0.001  & 2.92$\pm$0.03 	     &  -1.0$\pm$14.4    & $>$49	   & 167$\pm$2	  &	  -648$\pm$72	      &  -216$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs21}
\end{table*}



 
 


==> Tab_LAEs_CT-669.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around CT-669 (or ID=21).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  20:34:25.781    &  -35:37:36.46    & 11.6	      & 5134.99$\pm$0.03 & 3.224$\pm$0.001  & 2.26$\pm$0.04 	     &  -4.6$\pm$10.8    & $>$50	   & 314$\pm$6	  &	  426$\pm$72	      &  355$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs21}
\end{table*}



 
 


==> Tab_LAEs_CTS-C22.31.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around CTS-C22.31 (or ID=36).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  02:04:37.863    &  -45:59:16.16    & 25.7	      & 5162.95$\pm$0.03 & 3.247$\pm$0.001  & 3.66$\pm$0.03 	     &  -1.8$\pm$8.2    & $>$106	   & 221$\pm$2	  &	  71$\pm$72	      &  0$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs36}
\end{table*}



 
 


==> Tab_LAEs_Q-2204-408.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around Q-2204-408 (or ID=26).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  22:07:33.216    &  -40:37:00.16    & 12.8	      & 5077.85$\pm$0.03 & 3.177$\pm$0.001  & 31.40$\pm$0.07 	     &  -119$\pm$150    & $>$50	   & 98$\pm$4	  &	  -143$\pm$72	      &  -287$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs26}
\end{table*}



 
 


==> Tab_LAEs_Q-N1097.1.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around Q-N1097.1 (or ID=11).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  02:46:35.498    &  -30:04:35.22    & 26.9	      & 4981.82$\pm$0.03 & 3.098$\pm$0.001  & 2.92$\pm$0.03  	     &  -3.8$\pm$10.9	 & $>$65	   & 157$\pm$2    &	   -73$\pm$72	      &   1470$\pm$450	     \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs11}
\end{table*}



 
 


==> Tab_LAEs_Q2355+0108.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around Q2355+0108 (or ID=47).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  23:58:08.881    &  01:25:12.86     & 5.3	      & 5346.52$\pm$0.04 & 3.398$\pm$0.001  & 3.19$\pm$0.02          &  -1.9$\pm$11.0	 & $>$66	   & 129$\pm$1    &	   205$\pm$72	    &  889$\pm$450     \\
LAE2	 &  23:58:08.913    &  01:25:08.05     & 5.1	      & 5357.46$\pm$0.04 & 3.407$\pm$0.001  & 2.73$\pm$0.03          &  4.1$\pm$18.6	 & $>$151	   & 197$\pm$3    &	   819$\pm$72	    &  1504$\pm$450     \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs47}
\end{table*}



 
 


==> Tab_LAEs_SDSSJ0100+2105.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around SDSSJ0100+2105 (or ID=40).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  01:00:27.486    &  21:05:24.91     & 18.5 	      & 4964.80$\pm$0.03 & 3.084$\pm$0.001  & 6.37$\pm$0.03 	     &  -20.6$\pm$11.1    & $>$141	   & 116$\pm$1	  &	  -951$\pm$72	      &  -1170$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs40}
\end{table*}



 
 


==> Tab_LAEs_SDSSJ0219-0215.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around SDSSJ0219-0215 (or ID=43).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  02:19:39.060    &  -02:15:59.59    & 18.5	      & 4907.66$\pm$0.03 & 3.037$\pm$0.001  & 3.63$\pm$0.03 	     &  6.6$\pm$17.8    & $>$136	   & 202$\pm$2	  &	  74$\pm$72	      &  -371$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs43}
\end{table*}



 
 


==> Tab_LAEs_SDSSJ1209+1138.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around SDSSJ~1209+1138 (or ID=7).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$    & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$			  & $f_{\lambda}$				    & EW$_{\rm rest}$ & $\sigma_v$ &   $\Delta v_{\rm Neb}$   & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)  		  & (10$^{-20}$ cgs)				    & (\AA)	    & (km s$^{-1}$)&   (km s$^{-1}$)	      & (km s$^{-1}$)	       \\
\hline	 	 	 																							    
LAE1	 &  12:09:17.742    &  11:38:44.56     & 13.7	     & 5004.91$\pm$0.03 & 3.117$\pm$0.001  & 1.88$\pm$0.02  		     &  5.6$\pm$12.8				       & $>$81         & 137$\pm$3    &   -654$\pm$72		 &    0$\pm$450 	  \\
LAE2	 &  12:09:17.298    &  11:38:48.77     & 20.2	     & 5004.91$\pm$0.03 & 3.117$\pm$0.001  & 2.76$\pm$0.03  		     &  1.6$\pm$18.2				       & $>$420        & 172$\pm$2    &   -654$\pm$72		 &   -5$\pm$450 	  \\
LAE3	 &  12:09:17.623    &  11:38:54.89     & 24.2	     & 5023.15$\pm$0.03 & 3.132$\pm$0.001  & 3.02$\pm$0.03  		     &  3.9$\pm$14.2				       & $>$183        & 176$\pm$2    &    436$\pm$72		 & 1092$\pm$450 	  \\
LAE4	 &  12:09:16.759    &  11:38:47.85     & 24.6	     & 5029.23$\pm$0.03 & 3.137$\pm$0.001  & 3.13$\pm$0.03  		     & -9.8$\pm$10.2				       & $>$74         & 152$\pm$2    &    799$\pm$72		 & 1456$\pm$450 	  \\
LAE5	 &  12:09:19.090    &  11:38:17.78     & 21.0	     & 5012.21$\pm$0.03 & 3.123$\pm$0.001  & 2.53$\pm$0.03  		     & -8.6$\pm$11.4				       & $>$54         & 184$\pm$3    &   -218$\pm$72		 &  437$\pm$450 	  \\
\hline
\end{tabular}}
\flushleft{We list the coordinates and the distance $d$ (arcsec) from the quasar for each LAE discovered. For the Ly$\alpha$ emission-line in the spectrum of each LAE, we report 
the line center, the redshift, the line flux (in unit of 10$^{-17}$ erg s$^{-1}$ cm$^{-2}$), the underlying continuum flux $f_{\lambda}$ (in unit of 10$^{-20}$ erg s$^{-1}$ cm$^{-2}$ \AA$^{-1}$), the rest-frame equivalent width, 
and the line width as $\sigma_v$ of a Gaussian fit to the line. In addition, $\Delta v_{\rm Neb}$ and $\Delta v_{\rm QSO}$
are the velocity shift from the peak of the Ly$\alpha$ emission of the nebula and the systemic of the quasar targeted, respectively.
The uncertainty on the latter is dominated by the uncertainty on the systemic redshift of the quasar.
}
\label{tabLAEs7}
\end{table*}



 
 


==> Tab_LAEs_SDSSJ1429-0145.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around SDSSJ1429-0145 (or ID=20).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  14:29:02.011    & -01:45:14.14     & 16.6	      & 5386.63$\pm$0.04 & 3.431$\pm$0.001  & 3.12$\pm$0.03 	     &  -5.0$\pm$8.3     & $>$84	   & 259$\pm$3	  &	  407$\pm$72	      &  2456$\pm$450	 \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs20}
\end{table*}



 
 


==> Tab_LAEs_SDSSJ2358+0125.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around SDSSJ2358+0125 (or ID=28).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  23:58:08.905    &	01:25:11.64    & 5.4	      & 5346.52$\pm$0.04 & 3.398$\pm$0.001  & 3.10$\pm$0.09 	    &  5.3$\pm$13.6	& $>$132	   & 122$\pm$4	  &    205$\pm$72	      &  1576$\pm$450     \\
LAE2	 &  23:58:08.929    &	01:25:07.21    & 5.2	      & 5358.67$\pm$0.04 & 3.408$\pm$0.001  & 5.08$\pm$0.04 	    &  -5.0$\pm$25.4	& $>$45		   & 273$\pm$3	  &    887$\pm$72	      &  2261$\pm$450     \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs28}
\end{table*}



 
 


==> Tab_LAEs_TEX1033+137.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around TEX1033+137 (or ID=57).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 &  10:36:26.554    &	13:26:56.87    &  6.7	      & 4978.17$\pm$0.03 & 3.095$\pm$0.001  & 8.33$\pm$0.03	     &  -12.7$\pm$13.6   & $>$149	   & 280$\pm$1	 &   -146$\pm$72	      &  440$\pm$450     \\
LAE2	 &  10:36:27.405    &	13:26:42.61    &  12.7	      & 4976.95$\pm$0.03 & 3.094$\pm$0.001  & 3.70$\pm$0.03	     &  -6.7$\pm$ 30.3   & $>$30	   & 200$\pm$2	 &   -220$\pm$72	      &  367$\pm$450     \\
LAE3	 &  10:36:27.219    &	13:26:49.75    &  5.4	      & 4980.60$\pm$0.03 & 3.097$\pm$0.001  & 4.14$\pm$0.03	     &  -0.8$\pm$27.7    & $>$36	   & 240$\pm$2	 &   0$\pm$72	              &  587$\pm$450     \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs57}
\end{table*}



 
 


==> Tab_LAEs_UM683.tex <==
\begin{table*}
\caption{Information on the Ly$\alpha$ emission for the LAEs around UM683 (or ID=8).}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\hline
\hline
Object	 &  RA		    &  Dec	       & $d$          & Line Center	 & Redshift	    & $F_{\rm Ly\alpha}$     & $f_{\lambda}$	 & EW$_{\rm rest}$ & $\sigma_v$   &   $\Delta v_{\rm Neb}$    & $\Delta v_{\rm QSO}$   \\
	 & (J2000)	    &  (J2000)	       & (\arcsec)    & (\AA)		 &		    & (10$^{-17}$ cgs)       & (10$^{-20}$ cgs)	 & (\AA)	   & (km s$^{-1}$)&   (km s$^{-1}$)           & (km s$^{-1}$)	      \\
\hline	 	 	 															    					   
LAE1	 & 03:36:28.701     &  -20:19:24.97    & 27.0	      & 5023.15$\pm$0.03 & 3.132$\pm$0.001  & 1.10$\pm$0.02  	     &  -7.9$\pm$4.8 	 & $>$56	   & 112$\pm$3    &	   0$\pm$72	      &   0$\pm$450	     \\
LAE2	 & 03:36:27.484     &  -20:19:32.29    &  9.2	      & 5023.15$\pm$0.03 & 3.132$\pm$0.001  & 1.35$\pm$0.02  	     &  -4.4$\pm$5.1 	 & $>$64	   & 128$\pm$2    &	   0$\pm$72	      &   0$\pm$450	     \\
\hline
\end{tabular}}
\flushleft{As for Table~\ref{tabLAEs8}.
}
\label{tabLAEs8}
\end{table*}



 
 


==> Tab_fit_average_profile.tex <==

\begin{table}
\scriptsize
\caption{Fit of the average Ly$\alpha$ surface brightness profile.}
\centering
\begin{tabular}{lcccccccc}
\hline
\hline
Sample   &  \#     &  $\langle z_{\rm Ly\alpha} \rangle$	 &  $C_e^{\rm  \ \ a}$ & $r_h^{\rm \ \ a}$ & $\chi^{2 \ \ {\rm b}}_e$ & $C_p^{\rm  \ \ c}$ & $\alpha^{\rm  \ \ c}$ &  $\chi^{2 \ \ {\rm d}}_p$     \\
     &    &    & ($10^{-18}$)   & (kpc) & & ($10^{-18}$) & (kpc) &  \\
\hline
All & 60$^{\rm e}$ & 3.211 & 56.6 & 15.4 & 4.8 & 4103.7 & -1.90 & 35.1 \\
\hline
RQ$^{\rm f}$ & 40$^{\rm e}$ & 3.223 & 55.0 & 15.2 & 7.5 & 3596.5 & -1.88 & 33.5 \\
RL$^{\rm f}$ & 14 & 3.185 & 56.2 & 16.2 & 0.6 & 3240.4 & -1.81 & 45.2 \\
\hline
\end{tabular}
\label{Tab:profilesfit}
\flushleft{$^{\rm a}$ Best-fit parameters assuming SB profile ${\rm SB}(r)=C_e {\rm exp}(-r/r_h)$. $C_e$ is in unit of $10^{-18}$~erg~s$^{-2}$~cm$^{-2}$~arcsec$^{-2}$.}
\flushleft{$^{\rm b}$ Reduced chi square for the exponential fit.}
\flushleft{$^{\rm c}$ Best-fit parameters assuming SB profile ${\rm SB}(r)=C_p r^\alpha$. $C_p$ is in unit of $10^{-18}$~erg~s$^{-2}$~cm$^{-2}$~arcsec$^{-2}$.}
\flushleft{$^{\rm d}$ Reduced chi square for the power-law fit.}
\flushleft{$^{\rm e}$ PKS-1017+109 is not included.}
\flushleft{$^{\rm f}$ RQ and RL stand for radio-quiet and radio-loud. Note that 6 targets currently do not have information in radio.}
\end{table}
	


==> Tab_sample_MUSEUM.tex <==

\begin{table*}
\scriptsize
\caption{QSO MUSEUM: the sample.}
\centering
\begin{tabular}{lccccccccccc}
\hline
\hline
Quasar	& RA	& Dec	& $z_{\rm systemic}^{\rm a}$	& $z_{\rm peak\, Ly\alpha}^{\rm b}$ & $i_{\rm AB}^{\rm c}$ & Radio Flux$^{\rm d}$ & Seeing$^{\rm e}$ & Weather$^{\rm f}$ & Exp. Time$^{\rm g}$	& SB limit$^{\rm l}$ & ESO Programme \\	
	& (J2000) & (J2000) & & & (mag)	& (mJy) & (arcsec)	& 	& (min) & ($10^{-19}$~cgs)& \\
\hline
SDSS~J2319-1040   &  23:19:34.800	&  -10:40:36.00   &  3.166  &  3.172  & 18.17 & <0.396 & 1.40 & CL-WI   & 45.  	        &  8.2 & 094.A-0585(A) \\ %FAB: DONE! REDO PSF SUB - larger radius?
UM~24		  &  00:15:27.400	&  +06:40:12.00   &  3.133  &  3.163  & 17.08 & <0.396 & 1.62 & CL	 & 45.  	&  8.8 & 094.A-0585(A) \\ %FAB: DONE! REDO PSF SUB - larger radius?
J~0525-233	  &  05:25:06.500	&  -23:38:10.00   &  3.110  &  3.123  & 17.71 & 398.0* & 0.86 & CL	 & 45.  	&  8.5 & 094.A-0585(A) \\
Q-0347-383	  &  03:49:43.700	&  -38:10:31.00   &  3.219  &  3.230  & 17.63 & <0.210* & 1.40 & CL	 & 45.  	&  7.6 & 094.A-0585(A) \\
SDSS~J0817+1053   &  08:17:52.099	&  +10:53:29.68   &  3.320  &  3.336  & 18.08 & <0.381 & 1.47 & CL	 & 30.  	&  8.0 & 094.A-0585(A) \\ %there are cosmic rays as expected...remove them from NB image
SDSS~J0947+1421	  &  09:47:34.200	&  +14:21:17.00   &  3.029  &  3.073  & 17.04 & <0.423 & 1.21 & CL	 & 45.  	& 10.4 & 094.A-0585(A) \\ %big star nearby in NB: mask it! 
SDSS~J1209+1138	  &  12:09:18.000	&  +11:38:31.00   &  3.117  &  3.126  & 17.63 & <0.432 & 1.22 & CL	 & 45.  	&  8.5 & 094.A-0585(A) \\ %there are 2 nebulae...CHECK again if the second is real...
UM683		  &  03:36:26.900	&  -20:19:39.00   &  3.132  &  3.132  & 18.59 & <0.450* & 1.05 & CL-PH/PH-WI & 180.     &  5.0 & 094.A-0585(A)/095.A-0615(A) \\
Q-0956+1217	  &  09:58:52.200	&  +12:02:45.00   &  3.301  &  3.316  & 17.48 & <0.414& 1.12 & PH	 & 45.  	&  8.4 & 094.A-0585(A) \\
SDSS~J1025+0452	  &  10:25:09.600	&  +04:52:46.00   &  3.227  &  3.243  & 17.92 & <0.435& 1.10 & PH	 & 45.  	&  8.5 & 094.A-0585(A) \\
Q-N1097.1	  &  02:46:34.200	&  -30:04:55.00   &  3.078  &  3.099  & 18.81 & <0.180* & 1.18 & PH-HU   & 45.  	& 10.6 & 094.A-0585(A) \\
SDSS~J1019+0254	  &  10:19:08.255	&  +02:54:31.94   &  3.376  &  3.395  & 18.26 & <0.432 & 1.22 & PH-HU   & 45.  	        &  7.4 & 094.A-0585(A) \\
PKS-1017+109      &  10:20:10.000	&  +10:40:02.00   &  3.164  &  3.167  & 18.13 & <0.438 & 0.91 & PH-HU   & 45.  	        &  8.2 & 094.A-0585(A) \\
%		  &  10:20:10.000	&  +10:40:02.00   &  3.164  &  3.167  & & 0.66 & CL-PH   & 270.              &  & 096.A-0937(A) \\
SDSS~J2100-0641	  &  21:00:25.030  	&  -06:41:45.00   &  3.126  &  3.136  & 18.29 & <0.471 & 0.85 & CL	 & 45.  	& 10.5 & 095.A-0615(B) \\ %FAB: SOLVED!! there might be problems in removing three bright nearby sources
SDSS~J1550+0537	  &  15:50:36.806  	&  +05:37:50.07   &  3.141  &  3.147  & 18.08 & <1.458 & 1.01 & CL-WI   & 45.  	        & 10.2 & 095.A-0615(B) \\ %comment on the presence of the close-by galaxy (there is no nebular emission at that location)
SDSS~J2348-1041	  &  23:48:56.488   	&  -10:41:31.17   &  3.142  &  3.190  & 18.17 & <0.426 & 1.72 & CL-WI   & 45.  	        &  8.0 & 095.A-0615(B) \\
SDSS~J0001-0956	  &  00:01:44.886   	&  -09:56:30.83   &  3.340  &  3.348  & 18.56 & 50.25$^{\rm m}$ & 1.81 & PH-WI  & 45.  	&  7.8 & 095.A-0615(B) \\
SDSS~J1557+1540	  &  15:57:43.300	&  +15:40:20.00   &  3.265  &  3.288  & 18.46 & <0.429 & 0.81 & CL	 & 45.  	&  7.4 & 095.A-0615(A) \\ % rms calculation wrong...checked-->there is a bright star (select region for better calc)
SDSS~J1307+1230	  &  13:07:10.200	&  +12:30:21.00   &  3.188  &  3.229  & 17.58 & <0.408 & 0.89 & CL	 & 45.  	&  8.3 & 095.A-0615(A) \\
SDSS~J1429-0145	  &  14:29:03.033       &  -01:45:19.00   &  3.395  &  3.425  & 17.90 & <0.786 & 0.79 & CL	 & 45.  	&  7.7 & 095.A-0615(A) \\
CT-669		  &  20:34:26.300	&  -35:37:27.00   &  3.219  &  3.218  & 18.13 & <0.990* & 0.74 & CL	 & 45.  	& 11.9 & 095.A-0615(A) \\
Q-2139-4434	  &  21:42:25.900	&  -44:20:18.00   &  3.176  &  3.229  & 17.95 & --- & 1.02 & CL	 & 45.  	&  8.9 & 095.A-0615(A) \\
Q-2138-4427	  &  21:41:59.500	&  -44:13:26.00   &  3.061  &  3.142  & 18.13 & --- & 0.81 & CL	 & 45.  	&  7.7 & 095.A-0615(A) \\
SDSS~J1342+1702	  &  13:42:33.200	&  +17:02:46.00   &  3.062  &  3.053  & 18.55 & <0.414 & 1.03 & CL	 & 30.  	& 10.3 & 095.A-0615(A) \\
SDSS~J1337+0218	  &  13:37:57.900	&  +02:18:21.00   &  3.307  &  3.344  & 18.37 & <0.432 & 0.75 & CL-PH   & 45.  	& 14.2 & 095.A-0615(A) \\ %check this nebula...companions? bright emission at lower redshift
Q-2204-408	  &  22:07:34.300	&  -40:36:57.00   &  3.181  &  3.179  & 17.17 & --- & 0.84 & TN	 & 45.  	& 25.3 & 095.A-0615(A) \\ %FAB: SOLVED (worse depth than others)!! check this cube...qso stronger than expected...FAB: worse depth: there is small nebula and companion nebula
Q-2348-4025	  &  23:51:16.100	&  -40:08:36.00   &  3.318  &  3.334  & 17.98 & --- & 0.87 & CL	 & 45.  	&  7.2 & 095.A-0615(A) \\
SDSS~J2358+0125	  &  23:58:08.000 	&  +01:25:07.00   &  3.375  &  3.395  & 17.41 & <0.423 & 0.89 & CL	 & 45.  	& 10.8 & 095.A-0615(A) \\
Q-0042-269	  &  00:44:52.300	&  -26:40:09.00   &  3.344  &  3.350  & 19.10 & <0.060* & 0.80 & CL	 & 45.  	&  6.8 & 095.A-0615(A) \\ %check this nebula...bright narrow emission...also velocity map has problems
Q-0115-30 	  &  01:17:34.000	&  -29:46:29.00   &  3.180  &  3.221  & 17.95 & <0.540* & 0.91 & CL	 & 45.  	&  7.1 & 095.A-0615(A) \\
SDSS~J1427-0029	  &  14:27:55.800	&  -00:29:51.00   &  3.357  &  3.354  & 18.27 & <0.513 & 0.95 & CL	 & 45.  	& 17.1 & 095.A-0615(A) \\ %(not very good data) %check this cube...seems no nebula % one star to be removed from NB (to do profile...)
UM670		  &  01:17:23.300	&  -08:41:32.00   &  3.131  &  3.203  & 17.64 & <0.450 & 0.80 & CL	 & 45.  	&  7.5 & 095.A-0615(A) \\
Q-0058-292	  &  01:01:04.700	&  -28:58:03.00   &  3.069  &  3.101  & 18.53 & <3.570* & 1.42 & CL-WI   & 45.  	&  7.2 & 095.A-0615(A) \\
Q-0140-306	  &  01:42:54.700	&  -30:23:45.00   &  3.125  &  3.132  & 18.33 & 3.7*$^{\rm n}$ & 1.39 & CL-WI   & 45.  	&  8.3 & 095.A-0615(A) \\
Q-0057-3948	  &  00:59:53.200	&  -39:31:58.00   &  3.223  &  3.251  & 19.49 & <0.150* & 1.09 & CL-WI   & 45.  	&  9.2 & 095.A-0615(A) \\
CTS-C22.31	  &  02:04:35.500	&  -45:59:23.00   &  3.247  &  3.246  & 19.50 & --- & 1.18 & CL-WI   & 45.  	&  7.2 & 095.A-0615(A) \\
Q-0052-3901A	  &  00:54:45.400	&  -38:44:15.00   &  3.197  &  3.203  & 19.10 & 27.3*$^{\rm o}$ & 1.25 & CL-WI   & 45.  	&  7.2 & 095.A-0615(A) \\
UM672		  &  01:34:38.600 	&  -19:32:06.00   &  3.130  &  3.127  & 18.52 & 46.0* & 1.87 & CL/CL-WI	& 90.	&  7.2 &  095.A-0615(A)/096.A-0937(B) \\ %FAB: DONE! REDO PSF subtraction -- larger radius?
SDSS~J0125-1027   &  01:25:30.900	&  -10:27:39.00   &  3.348  &  3.319  & 18.24 & <0.438 & 0.74 & CL	 & 45.  	&  7.3 & 095.A-0615(A) \\ %check this cube...bright narrow emission
SDSS~J0100+2105	  &  01:00:27.661	&  +21:05:41.57   &  3.100  &  3.097  & 18.15 & <2.22* & 0.73 & PH	 & 45.  	&  9.5 & 095.A-0615(A) \\
SDSS~J0250-0757	  &  02:50:21.800	&  -07:57:50.00   &  3.342  &  3.336  & 18.19 & <0.471 & 0.67 & PH	 & 45.  	&  7.5 & 095.A-0615(A) \\
SDSS~J0154-0730	  &  01:54:40.328	&  -07:30:31.85   &  3.321  &  3.337  & 18.66 & <0.399 & 0.75 & PH	 & 45.  	&  6.7 & 095.A-0615(A) \\
SDSS~J0219-0215	  &  02:19:38.732	&  -02:15:40.47   &  3.042  &  3.036  & 18.29 & <0.492 & 0.64 & PH	 & 45.  	&  9.3 & 095.A-0615(A) \\
CTSH22.05	  &  01:48:18.130	&  -53:27:02.00   &  3.087  &  3.127  & 18.66 & --- & 1.34 & CL-WI   & 45.  	&  7.5 & 096.A-0937(B) \\
SDSS~J2321+1558	  &  23:21:54.980	&  +15:58:34.24   &  3.197  &  3.241  & 18.29 & <1.770* & 1.61 & CL	 & 45.  	&  7.7 & 096.A-0937(B) \\
FBQS~J2334-0908   &  23:34:46.400	&  -09:08:12.24   &  3.312  &  3.361  & 17.96 & 27.65 & 1.18 & CL	 & 45.  	&  7.3 & 096.A-0937(B) \\
Q2355+0108	  &  23:58:08.540	&  +01:25:07.20   &  3.385  &  3.395  & 17.61 & <0.423 & 1.23 & CL	 & 45.  	&  7.4 & 096.A-0937(B) \\
6dF~J0032-0414	  &  00:32:05.380	&  -04:14:16.21   &  3.156  &  3.162  & 18.88 & 34.55 & 1.59 & CL	 & 45.  	&  9.6 & 096.A-0937(B) \\
UM679		  &  02:51:48.060	&  -18:14:29.00   &  3.197  &  3.215  & 18.77 & <1.020* & 0.96 & PH	 & 45.  	&  7.0 & 096.A-0937(B) \\
PKS0537-286	  &  05:39:54.267       &  -28:39:56.00   &  3.109  &  3.141  & 18.93 & 862.2* & 0.74 & PH	 & 45.  	&  6.7 & 096.A-0937(B) \\
SDSS~J0819+0823	  &  08:19:40.580	&  +08:23:57.98   &  3.197  &  3.205  & 18.33 & <0.423 & 0.73 & PH	 & 45.  	&  7.7 & 096.A-0937(B) \\
SDSS~J0814+1950	  &  08:14:53.449       &  +19:50:18.62   &  3.138  &  3.137  & 18.74 & 4.45 & 0.75 & PH	 & 45.  	& 10.2 & 096.A-0937(B) \\ %FAB: DONE!  REDO PSF subtraction!! too much subtracted!
SDSS~J0827+0300	  &  08:27:21.968       &  +03:00:54.74   &  3.144  &  3.137  & 18.09 & 7.64 & 0.96 & CL	 & 45.  	&  7.8 & 096.A-0937(B) \\
SDSS~J0905+0410	  &  09:05:49.058       &  +04:10:10.15   &  3.149  &  3.165  & 19.73 & 194.64 & 0.93 & CL	 & 45.  	&  7.1 & 096.A-0937(B) \\
S31013+20	  &  10:16:44.319       &  +20:37:47.29   &  3.109  &  3.108  & 19.19 & 727.01 & 0.92 & PH	 & 45.  	&  7.9 & 096.A-0937(B) \\
SDSS~J1032+1206	  &  10:32:12.886       &  +12:06:12.83   &  3.188  &  3.195  & 18.66 & 2.29 & 0.89 & CL-WI   & 45.  	&  7.7 & 096.A-0937(B) \\
TEX1033+137	  &  10:36:26.886       &  +13:26:51.75   &  3.089  &  3.097  & 18.09 & 102.52$^{\rm p}$& 0.70 & PH	 & 45.  	&  9.0 & 096.A-0937(B) \\
SDSS~J1057-0139	  &  10:57:13.250    	&  -01:39:13.79   &  3.406  &  3.452  & 18.40 & 21.13 & 1.31 & PH	 & 45.  	& 11.2 & 096.A-0937(B) \\ %check this nebula...might be that the nebula is at lower z than expected (do dlower cut?)
Q1205-30	  &  12:08:12.730	&  -30:31:07.00   &  3.037  &  3.047  & 17.95 & <0.660* & 0.63 & PH	 & 45.  	&  9.2 & 096.A-0937(B) \\
LBQS1244+1129	  &  12:46:40.370       &  +11:13:02.92   &  3.118  &  3.157  & 18.19 & <0.408 & 1.45 & PH	 & 45.  	&  9.8 & 096.A-0937(B) \\
SDSS~J1243+0720   &  12:43:53.960       &  +07:20:15.47   &  3.183  &  3.178  & 19.16 & 2.29 & 1.29 & PH	 & 45.  	&  8.5 & 096.A-0937(B) \\
LBQS1209+1524	  &  12:12:32.040       &  +15:07:25.63   &  3.061  &  3.075  & 18.02 & <0.450 & 1.42 & PH	 & 45.  	&  8.9 & 096.A-0937(B) \\
%Q-1346+001	  &  13:49:17.800	&  -00:07:03.00   &   &         & & 0.88 & CL      &  &  095.A-0615(A) \\ It's a star!!
\hline
\end{tabular}
\label{tab:sample}
\flushleft{$^{\rm a}$ Systemic redshift of the quasar evaluated from the peak of the {\bf C~IV} line, correcting for the expected shift as estimated by {\bf Shen et al. 2016}. The
intrinsic uncertainty on this correction is $\sim415$~km~s$^{-1}$ and dominate the error badget ($\Delta z\approx0.007$).}
\flushleft{$^{\rm b}$ Estimated as flux-weighted centroid of the Ly$\alpha$ emission for a circular aperture with a diameter of $3\arcsec$ and centered on the peak of the SB map of
each nebula.} 
\flushleft{$^{\rm c}$ Extracted from the final MUSE datacubes using the SDSS filter transmission curve and a circular aperture with a diameter of $3\arcsec$. The average uncertainty on
this magnitude is $\sim5\%$.}
\flushleft{$^{\rm d}$ We report the integrated flux at 1.4~GHz from the FIRST survey ({\bf add reference to Becker}) for northern sources, while the peak flux at 1.4~GHz from {\bf add ref} for the southern sources (indicated by *). For sources with Dec$<-40$ (and thus not
covered by NVSS) we report the from {\bf add ref}. For the non-detections, and thus radio-quiet objects, we report the $3\times rms$ in mJy/beam from each catalogue.} 
\flushleft{$^{\rm e}$ Seeing computed from the ``white-light'' image of the final MUSE datacubes as FWHM of a Moffat profile.} %FAB: beta parameter for the moffat is between 2.15 and 3.45 (see my paper for discussion on this...)
\flushleft{$^{\rm f}$ Sky conditions during observations as from the ESO observations log: PH-photometric; CL-clear; WI-windy; TN-thin cirrus; HU-humid}
\flushleft{$^{\rm g}$ Exposure time on source (without overheads).}
\flushleft{$^{\rm l}$ For each combined datacube, we list the $2\sigma$ surface brightness limit computed for the layer (1.25\AA) at the redshift of the Ly$\alpha$ emission (column 5 here) and within an aperture of 1 arcsec$^{2}$. The cgs units are erg~s$^{-1}$~cm$^{-2}$~arcsec$^{-2}$.}
\flushleft{$^{\rm m}$ The radio source is at $\approx13.5\arcsec$ from the quasar (see {\bf appendix ??}).}
\flushleft{$^{\rm n}$ The radio source is at $\approx8\arcsec$ from the quasar ({\bf cite NVSS}).}
\flushleft{$^{\rm o}$ The radio source is at $\approx2.3\arcsec$ from the quasar ({\bf cite NVSS}).}
\flushleft{$^{\rm p}$ This source is a radio galaxy with two lobes separated by $\approx8.5\arcsec$ (see {\bf appendix ??}). We report the sum of the integrated flux of the two lobes.} 
\end{table*}
	

